Evaluating Answer Reranking Strategies in Time-sensitive Question Answering

Despite advancements in state-of-the-art models and information retrieval techniques, current systems still struggle to handle temporal information and to correctly answer detailed questions about past events. In this paper, we investigate the impact of temporal characteristics of answers in Question Answering (QA) by exploring several simple answer selection techniques. Our findings emphasize the role of temporal features in selecting the most relevant answers from diachronic document collections and highlight differences between explicit and implicit temporal questions.

==> related_work.tex <==
\section{Background and Related Work}
%Temporal information 

%Temporal information is an important characteristic embedded in documents; thus, it is very crucial to analyze such information in documents. 
In recent years, utilizing temporal information of text has gained much attention as it can improve the performance of multiple tasks like event occurrence time prediction \cite{Wang2021EventOD}, web search \cite{stack2006full,Temporal_QA_Nugget}, timeline summarization \cite{steen2019abstractive,tran2015timeline}, and question answering \cite{wang2020answering,shang2022improving}.

Several works have been proposed on utilizing temporal information in question answering. For example, \cite{jia2018tequila} address temporal QA problem over knowledge graphs. The authors decompose questions into non-temporal sub-questions and temporal constraints. They rely on hand-crafted rules to tackle temporal information. Similarly, \cite{Temporal_QA_Question_Decompose} decompose complex questions into simpler ones and use embedded temporal expressions in the questions as well as demonstrate the effects of the temporal layer. \cite{Temporal_QA_Temp_Inference} propose a QA methodology that draws temporal inference based on semantic inference between events, entities, and their definition, along with extracting relations between events and temporal expression in question or expected answers.
In \cite{Temporal_QA_Nugget}, events are captured from offline documents and assigned by a specific entity containing the corresponding dates. As a result, the questions are answered by matching captured events instead of retrieving top-related documents. While each of these works uses temporal aspects, none use the timestamp information obtained from document metadata.

On the other hand, several works have been proposed focusing on temporal ranking of documents \cite{Alonso,TemporalInfoSurvey,types_time_retrieval,kanhabua2011ranking}. For example, \cite{TimeLangModel} and \cite{recency_relevance} use document metadata when calculating temporal score by favoring the recency of retrieved documents for short queries or web searches and then combining with the relevance score. Thus the documents are re-ranked by the combined score. \cite{li2003time} proposed a time-based language model that gives preference to the most recent documents by considering the timestamp metadata of the documents. Other research works focus on considering the time period mentioned in the question for ranking the relevant documents. \cite{arikan2009time} propose a retrieval framework that takes into account the temporal expressions of document. This research work assumes queries to contain temporal expressions explicitly. Further, in \cite{Temporal_IR_Query_Time}, implicit temporal queries are mapped to a time period by using a temporal language model and keyword frequency by a specific period of time, or by using the distribution of retrieved documents by obtaining timestamps. After then, by using a decay function, documents retrieved around the query time scope are favored by calculating a temporal score, which is then combined with a relevance score. Whereas in \cite{metzler2009improving} proposed a method to re-rank documents by analyze frequency of query logs over time for temporal implicit queries. This method is typical applied for web search, where query log information is available. 
\cite{zhou-etal-2021-temporal} propose distant supervision model for temporal reasoning over Implicit and explicit events.

Despite the similarity between our proposed work and the listed works, few works apply question answering on long-term document collections such as news or web archives. Our work is most related to \cite{QANA}, where the re-ranking mechanism is implemented on retrieved paragraphs by utilizing a time-aware re-ranking module. Specifically, temporal information can be extracted from the question itself for explicitly time-scoped questions, or it can be drawn from the distribution of relevant documents over time for implicitly time-scoped questions. The temporal information is then used to calculate a temporal score which is combined with a relevance score to re-rank retrieved documents. This research aims to expand the scope by re-ranking modules on both retrieved documents and extracted answers and employing supervised methods.


==> taskformulation_old.tex <==
\vspace{-3mm}
\section{Motivating Example}
\vspace{-3mm}
To illustrate the problem, let us consider a hypothetical scenario where a user's question about some past event has five possible candidate answers, each with a different temporal distribution that are depicted in Figure \ref{fig:AnswerDistribution}. For simplicity, let us assume that the event date is explicitly mentioned in the question and the reader component (or RAG-based model) of the QA system assigns equal scores to all the candidate answers. 
The temporal distribution of the answers is as follows:
\vspace{-3mm}
\begin{itemize}
    \item Answer \textbf{\emph{A}} is the most common however the documents that contain it were published before the event date.
    \item Answer \textbf{\emph{B}} appears around the time of the event.
    \item Answer \textbf{\emph{C}} is uniformly distributed across the time.
    \item Answer \textbf{\emph{D}} is the most commonly occurring answer after the event.
    \item Answer \textbf{\emph{E}} is the most recent answer, though infrequent.
\end{itemize}


\begin{figure}[!t]
\centering
\includegraphics[width=.7\textwidth]{figures/answer_distribution2.pdf}
\caption{An example temporal distribution of candidate answers. The date of the queried event is indicated by the red cross mark on timeline.} \label{fig:AnswerDistribution}
\end{figure}

\vspace{-3mm}

Each candidate answer offers a unique advantage. 
For example, Answer \textbf{\emph{A}} seems to be a good candidate based on its overall frequency - a strategy often used in answer post-processing and final answer selection in QA systems \cite{zhu2021retrieving}. 
Answer \textbf{\emph{B}}, being temporally close to the event, might be more relevant for answering specific details about the event itself, which may not be reported afterwards. Answer \textbf{\emph{D}}, appearing after the event, may offer valuable retrospective insights or account for any novel information that emerged after the event, though, it may lack immediate or accurate details. Similarly, Answer \textbf{\emph{E}} as the most recent answer, might provide the most up-to-date information, but its low frequency raises concerns about its reliability. Lastly, Answer \textbf{\emph{C}} might be a good candidate as its uniformly distributed across time. We note that these are just extreme cases and in reality there are different degrees of the combinations of them. Nevertheless, the question as to what extent the temporal positions of answers matter in relation to the occurrence dates of queried events is still open.

%We also note that while the above example assumes that the question explicitly states the event's date, many questions on past events may lack temporal references. This adds complexity to selecting the correct answer\footnote{One could try to infer the actual event time by analyzing retrieved documents as, for example, in \cite{QANA}.}. In this paper, we study both the cases of questions explicitly stating dates of queried events and questions without any such temporal signals. 

Investigating temporal answer distributions in diachronic document collections could present valuable opportunities for improving the accuracy and robustness of open-domain QA systems implemented over such document corpora. 

